DeepReDuce: ReLU Reduction for Fast Private Inference

The recent rise of privacy concerns has led researchers to devise methods for private neural inference -- where inferences are made directly on encrypted data, never seeing inputs. The primary challenge facing private inference is that computing on encrypted data levies an impractically-high latency penalty, stemming mostly from non-linear operators like ReLU. Enabling practical and private inference requires new optimization methods that minimize network ReLU counts while preserving accuracy. This paper proposes DeepReDuce: a set of optimizations for the judicious removal of ReLUs to reduce private inference latency. The key insight is that not all ReLUs contribute equally to accuracy. We leverage this insight to drop, or remove, ReLUs from classic networks to significantly reduce inference latency and maintain high accuracy. Given a target network, DeepReDuce outputs a Pareto frontier of networks that tradeoff the number of ReLUs and accuracy. Compared to the state-of-the-art for private inference DeepReDuce improves accuracy and reduces ReLU count by up to 3.5% (iso-ReLU count) and 3.5$\times$ (iso-accuracy), respectively.

==> 06Generality.tex <==
\section{Generality of DeepReDuce} \label{sec:Generality}
In this section we show DeepReDuce generalizes beyond ResNets and does not depend on residual connections.
Note that VGG16 was shown in Section~\ref{sec:ExperimentalResults},
here we provide additional analysis for completeness.

{\bf Effect of residual connections:} \textcolor{red}{
We first examine the impact of ResNets' residual connections 
%(present in ResNet \cite{he2016deep}) 
on the efficacy of DeepReDuce. 
We removed all the residual connections in ResNet18 (student network) and evaluate the stage-wise ReLU criticality, the first step in DeepReDuce. 
We then perform KD using both a residual teacher (Full-ReLU ResNet18) and a non-residual teacher network for a complete evaluation of impact of residual connections on ReLUs' criticality. 
Results are shown in Table \ref{tab:CriticalityNonRes}.} 
\textcolor{red}{
The accuracy degradation is substantial and varies with the position of ReLUs in the networks. 
When KD is performed with non-residual teacher, the recovered accuracy is less than KD with a residual teacher. 
Nonetheless, the (relative) criticality order of non-residual ResNet18 is same as residual ResNet18  (Table \ref{tab:ReluHeteroR18}). } 


\input{Tables/40Table_ReLUCriticalityNonRes}



{\bf DeepReDuce on MobileNets:} 
\textcolor{red}{Next, we examine the effectiveness of DeepReDuce on MobileNetV1 \cite{howard2017mobilenets}.
We chose to study MobileNet as it is very differenct from ResNet---the convolution layers
do not use residuals and the Depthwise architecture is FLOP optimized, which we believe is a poor match for DeepReDuce's ReLU minimization objective.
%types (a non-residual network with FLOPs-optimized Depthwise separable convolution) are significantly different than that of ResNet models.
We first evaluate the ReLUs' criticality (see Table \ref{tab:CriticalityInMobileNets} in Appendix \ref{SecAppendix:ParetoPointsMV1}) and then compare the performance of DeepReDuce models with conventionally (channel/fmap-resolution) scaled MobileNetV1. 
Results are shown in Figure \ref{fig:ParetoFrontierMV1} and the optimization steps for all DeepReDuce models are listed in Table \ref{tab:ParetoPointsMV1} in Appendix \ref{SecAppendix:ParetoPointsMV1}. 
The substantial gain (reduction) in accuracy (ReLU count) at iso-ReLU (iso-accuracy) shows the effectiveness of DeepReDuce ReLU optimization on MobileNetV1 \fixme{add numbers here? sounds generic.}.
 }

\textcolor{red}{
Thus, while residual connections benefit DeepReDuce, they are not
a necessity as DeepReDuce also performs well when residual connections are eliminated from the network and the non-residual networks such as MobileNets and VGG16 (Figure \ref{fig:ParetoFrontierVGG16}).}



%First, we evaluate the criticality of ReLUs in MobileNets (V1 \cite{howard2017mobilenets} and V2 \cite{sandler2018mobilenetv2}) on the CIFAR-100 and computed the stage-wise criticality metric $C_k$ (Eq. \ref{eqn:CriticalityMetric}). The results are shown in Table \ref{tab:CriticalityInMobileNets}.  We observed the similar trend as ResNet18 and ResNet34 on CIFAR-100/TinyImageNet (shown in Tables \ref{tab:ReluHeteroR18} and \ref{tab:ResNetBlockDropout}), accuracy differs significantly across stages and $S_1$ ($S_4$) ReLUs are least (most) critical.

%\textcolor{red}{
%Further, to examine the efficacy of DeepReDuce on MobileNetV1, we compare the performance of DeepReDuce models with the conventionally (channel/fmap-resolution) scaled MobileNetV1. Results are shown in Figure \ref{fig:ParetoFrontierMV1} and the optimization steps for all the DeepReDuce models are listed in Table \ref{tab:ParetoPointsMV1} in Appendix \ref{SecAppendix:ParetoPointsMV1}. The substantial gain (reduction) in accuracy (ReLU count) at iso-ReLU (iso-accuracy) shows the effectiveness of DeepReDuce ReLU optimization on MobileNetV1  whose architecture and convolution types (a non-residual network with FLOPs-optimized Depthwise separable convolution) are significantly different than that of ResNet models. }






%{\bf DeepReDuce vs. conventional scaling in MobileNets}

==> Plots/15Figure_DesignSpace.tex <==
\begin{figure}[t] \centering
\includegraphics[scale=0.55]{Figures/DesignSpace}
\caption{Design space reduction in successive iterations of DeepReDuce: each iteration has its own design space which is reduced through subsequent steps of ReLU optimization. Three points in Step 3 represents the three scaled networks with different ReLU counts.}
\label{fig:DesignSpace}
\end{figure}

==> Plots/16Figure_StageWiseReluPercentage.tex <==
\begin{figure}[t] \centering
\includegraphics[scale=0.225]{Figures/StageWiseReluPercentage}
\vspace{-2em}
\caption{Stage-wise ReLU distribution in CNNs: MV1/MV2 is MobileNetV1/V2.
We note most ReLUs go to the initial stages.}
\label{fig:StageWiseReluPercentage}
\end{figure}


==> Plots/22Figure_SAFENetLayerwiseComp.tex <==
\begin{figure}[t] \centering
\includegraphics[scale=0.15]{Figures/Safenet_layerwise_comp}
\vspace{-1em}
\caption{Layer-wise approximation/pruned-ReLUs in SAFENet and DeepReDuce models (iso-ReLU and iso-accuracy).  
}
\vspace{-1em}
\label{fig:SafenetLayerwiseComp}
\end{figure}


==> Tables/26Table_ReluScaling.tex <==
\begin{table} [htbp]
\caption{ReLU scaling in stage 2 of ``DeepReDuce''}
\label{tab:ReluScaling}
\centering 
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{ p {2.5cm} |c } 
 \toprule
 {\bf Scaling methods} &  $Net \text{(DR)}$  \\ \toprule
 Channel scaling by $\alpha$ &   $Net (\alpha\hat{\phi}, \alpha^2\Psi, \alpha^2\Gamma, \hat{l_{r}}, \hat{b_{r}}, \hat{s_{r}}, \hat{l_{nr}}, \hat{b_{nr}}, \hat{s_{nr}})$ \\ \midrule
 Fmap scaling by $\rho$   &   $Net (\rho^2\hat{\phi}, \Psi, \rho^2\Gamma, \hat{l_{r}}, \hat{b_{r}}, \hat{s_{r}}, \hat{l_{nr}}, \hat{b_{nr}}, \hat{s_{nr}})$\\ \midrule
 Layer-wise ReLU dropout (2:1)  &   $Net (\frac{\hat{\phi}}{2}, \Psi,  \Gamma, \frac{\hat{l_{r}}}{2}, \hat{b_{r}}, \hat{s_{r}}, L-\frac{\hat{l_{r}}}{2}, \hat{b_{nr}}, \hat{s_{nr}})$\\ \midrule
 Scaling \#Blocks in ReLU-stages (2:1) & $Net (\frac{\hat{\phi}}{2}, < \Psi,  < \Gamma, \frac{\hat{l_{r}}}{2}, \frac{\hat{b_{r}}}{2}, \hat{s_{r}}, L-\hat{l_{r}}, B-\hat{b_{r}}, \hat{s_{nr}})$ \\ 
 \bottomrule
\end{tabular} }

\end{table}


==> Tables/31Table_ResNet18MergedLayers.tex <==
\begin{table} [htbp]
\caption{Performance comparison for the network with merged non-ReLU layers(with ReLU-layer) }
\label{tab:MergedLayerComp}
\centering 
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|cc|cc} 
 \toprule
\multirow{2}{*}{\bf Network } & \multirow{2}{*}{\bf \#Conv } & \multirow{2}{*}{\bf \#ReLU } & \multicolumn{2}{c}{\bf CIFAR-100 } \\
& & & {\bf w/o kD} & {\bf w/ KD} \\
 \toprule
ResNet18(FR) & 17 & 557.06K & 74.46 & \\
$Arch1 \rightarrow$ResNet18  & 17 & 311.3K & 73.72 & 74.81 \\
$Arch2 \rightarrow$ResNet18 & 9 & 311.3K & 73.33 & 75.96 \\
\bottomrule
\end{tabular}}

\end{table}


==> Tables/40Table_ReLUCriticalityNonRes.tex <==
\begin{table} [t] \centering
\caption{Stage-wise criticality evaluation of ResNet18 with all the residual connections removed on CIFAR-100. We perform distillation with residual/non-residual teacher (ResNet18).  The accuracy degradation due to the elimination of residual connections is significant; however, criticality order remains same as in Table \ref{tab:ReluHeteroR18}.}
\label{tab:CriticalityNonRes} 
\resizebox{.5\textwidth}{!}{
\begin{tabular}{ccccccc} \toprule
\multirow{2}{*}{Stages} & \multirow{2}{*}{\#ReLUs} & \multirow{2}{*}{W/o KD} & \multicolumn{2}{c}{Residual Teacher} & \multicolumn{2}{c}{Non-residual Teacher} \\
\cmidrule(lr{0.5em}){4-5}  
\cmidrule(lr{0.5em}){6-7} 
& & & W/ KD (\%) & $C_k$  & W/ KD (\%) & $C_k$ \\ \toprule
%FR & 411.6K & 67.58 & - &    -   &425.6K & 68.46 & -     &  - \\ 
$S_1$ & 262.14K & 54.35($\downarrow$7.55\%) & 54.71($\downarrow$5.14\%) & 0.00 & 55.90($\downarrow$3.95\%) & 0.00 \\
$S_2$ & 131.07K & 61.83($\downarrow$5.80\%) & 64.37($\downarrow$4.42\%) & 6.87 & 64.47($\downarrow$4.32\%) & 6.40 \\
$S_3$ & 65.54K & 64.40($\downarrow$3.00\%) & 67.01($\downarrow$2.89\%) & 9.18 & 66.65($\downarrow$3.25\%) & 8.01 \\
$S_4$ & 32.77K & 56.81($\downarrow$2.09\%) & 61.10($\downarrow$2.06\%) & 5.01 & 60.63($\downarrow$2.53\%) & 3.55 \\  \bottomrule
\end{tabular} }
\end{table}


